On the Feasibility of Passive Bistatic ISAC Based on Unmodified LoRa

Integrated Sensing and Communication (ISAC) enables sensing capabilities by reusing communication signals, making it particularly attractive for large-scale deployments through signals of opportunity. While most existing ISAC research targets wideband systems, Low Power Wide Area Network (LPWAN) technologies such as LoRa remain largely unexplored from a radar-like sensing perspective. Existing LoRa-based approaches mainly focus on motion detection or require modifications of the communication waveform, limiting their applicability in deployed networks. This paper investigates the feasibility of radar-like sensing using unmodified LoRa communication signals as signals of opportunity in a purely passive bistatic ISAC configuration. The proposed approach focuses on Doppler-based sensing to enable target separation and super-resolved target estimation without interfering with existing LoRa network operation. The analytically derived sensing capabilities are compared against simulation results and validated through bistatic measurements using two USRP B210 software-defined radios, confirming the feasibility of Doppler-based LoRa sensing under practical conditions and revealing relevant implementation challenges. The results demonstrate that LoRa-based ISAC enables highly scalable, large-area, low-resolution sensing by leveraging existing infrastructure, providing a complementary sensing capability to area-limited high-resolution 6G ISAC systems, and a foundation for future multi-node and data fusion extensions.

==> texfiles/01_Related_Work.tex <==
\section{Related Work}
\label{sec:RelatedWork}

Integrated sensing and communication (ISAC) has recently gained significant attention in the context of low-power wide-area networks (LPWANs), primarily due to their dense deployment and large coverage. In contrast to high-bandwidth communication systems, LPWAN-based ISAC typically relies on passive sensing using signals of opportunity, as this enables sensing capabilities without impacting existing network operation. Similar strategies have also been explored in other IoT technologies, for instance by exploiting channel state information (CSI) in WiFi-based sensing systems.

Among LPWAN technologies, LoRa has emerged as the dominant platform for sensing-related research, owing to its widespread adoption and chirp spread spectrum modulation. Existing LoRa-based sensing approaches can be broadly categorized into two classes. The first class focuses on motion detection and classification, including applications such as respiration monitoring, human presence detection, and gait recognition, often using CSI or phase-based features combined with machine learning techniques. The second class addresses radar-like range estimation, typically through matched filtering or compressed sensing approaches. An overview of representative publications is provided in Table~\ref{table:ICAS_Papers}.

Despite these efforts, current LoRa-based sensing research exhibits several limitations. Motion-centric approaches do not aim at radar-like parameter estimation, while range-focused studies are predominantly simulation-based, often assume unrealistically large bandwidths, or rely on modified waveforms that are incompatible with operational LoRa networks. Moreover, a systematic analysis linking fundamental sensing limits, simulation-based feasibility, and experimental validation using unmodified LoRa communication signals is currently missing.

In this work, we address this gap by investigating Doppler-based radar-like sensing using unmodified LoRa signals in a bistatic ISAC configuration. By explicitly considering theoretical limits, simulation results, and practical measurement constraints, this paper provides a realistic assessment of the sensing potential and challenges of LoRa-based ISAC.


%
\begin{table}[t]
\caption{Publications on LoRa-based \ac{ISAC}}
\centering
% \setlength{\tabcolsep}{8pt}
\begin{tabularx}{0.96\linewidth}{l c c c}
\toprule
Reference	&	Motion detection		&	Classification		&	Range estimation		\\
\midrule
\cite{10.1145/3749522}	&	\checkmark	&		&		\\
\cite{Through_wall_sensing}	&	\checkmark	&		&		\\
\cite{chang2023explorationintegratedsensingcommunication}	&	\checkmark	&	\checkmark	&		\\
\cite{10.1145/3680207.3723478}	&	\checkmark	&		&		\\
\cite{10686583}	&	\checkmark	&	\checkmark	&		\\
\cite{11007496}	&		&		&	\checkmark	\\
\cite{HUANG2024155559}	&		&		&	\checkmark	\\
\cite{10.1007/978-981-96-1777-7_71}	&		&		&	\checkmark	\\
\bottomrule
\end{tabularx}
\label{table:ICAS_Papers}
\end{table}
%

